Efficiently Computing Provenance Graphs for Queries with Negation

Explaining why an answer is in the result of a query or why it is missing from the result is important for many applications including auditing, debugging data and queries, and answering hypothetical questions about data. Both types of questions, i.e., why and why-not provenance, have been studied extensively. In this work, we present the first practical approach for answering such questions for queries with negation (first-order queries). Our approach is based on a rewriting of Datalog rules (called firing rules) that captures successful rule derivations within the context of a Datalog query. We extend this rewriting to support negation and to capture failed derivations that explain missing answers. Given a (why or why-not) provenance question, we compute an explanation, i.e., the part of the provenance that is relevant to answer the question. We introduce optimizations that prune parts of a provenance graph early on if we can determine that they will not be part of the explanation for a given question. We present an implementation that runs on top of a relational database using SQL to compute explanations. Our experiments demonstrate that our approach scales to large instances and significantly outperforms an earlier approach which instantiates the full provenance to compute explanations.

==> gp-model.tex <==
\BG{DEAL OF THIS SECTION:
\textbullet Schema definition and the like 
            (We use $\schema(R)$ to denote the schema of relation $R$.)

\textbullet Introduce datalog 
\textbullet introduce relevant background SLD resolution and games
\textbullet Discuss evaluation variants?

\textbullet Introduce basic game theoretic notions?

\textbullet Review Semirings and M-semirings here?
}

% TODO:
% TODO: Introduce PG as shorthand for provenance graph
% TODO: Standardize on Datalog vs. datalog

\section{Provenance Games}
\label{sec:gp}

\emph{Provenance Games} as introduced by K\"ohler et al.~\cite{KL13} % are a crude
% way to
provide explanations $\explainq(P,Q(t),I)$ for all atoms $Q(t)$ in non-recursive \datalogneg programs $P$.
%Provenance games introduced by K\"ohler et al.~\cite{KL13} are constructed for a FO query expressed in non-recursive Datalog$^\neg$
%%an input query $Q$ (currently provenance game model supports non-recursive Datalog) 
%and a database instance $I$. 
%These games model evaluation (SLD resolution) of query $Q$ over $I$ as a 2-player game in a game-theoretic sense.
These games model evaluation of a query $Q$ over  $I$ as a 2-player game resembling SLD(NF) resolution. Such games contain positive and negative tuple nodes which represent claims about the existence of tuples in the database (\emph{EDB} in Datalog terminology) or query result (\emph{IDB} in Datalog terminology). \emph{Tuple nodes} are connected via \emph{rule nodes} and \emph{goal nodes}. These nodes represent successful (or failed) instantiations of the query's rules and the body goals in these rules. 
A game starting at a node for a tuple $\rel{R}(t)$ (predicate $\rel{R}$) corresponds to an argument between the two players where the player starting in that node is trying to prove the claim that $\rel{R}(t)$ exists while the opponent tries to refute this claim. Players take turns making moves (choosing outgoing edges from the current position in the game graph) until a sink position without outgoing edges is reached. The player  in this position looses the game. 
%\begin{Example}
For instance, 
Fig.~\ref{fig:exam-pg-why-NY-seattle} shows part of the provenance game for the query $Q$ from the running example. 
%Note that we abbreviate person names as $\cnst{j}$, $\cnst{p}$, $\cnst{m}$, and $\cnst{a}$. 
\emph{Tuple nodes} are shown as ovals while rule and goal nodes are shown as rectangles. 
To prove that Seattle can be reachable from New York with one transfer, the player trying to prove this fact starts in $\rel{Q}(n,s)$ and moves to one of the \emph{rule nodes}. %[connected to this position]. 
This corresponds to the claim that this particular rule instantiation is successful e.g., the player may move to $r_0(n,s,w)$, and claim that the rule instantiation $\rel{Q}(n,s) \dlImp \rel{Train}(n,w), \rel{Train}(w,s)$ is satisfied over $I$. The opponent responds by claiming that a goal in the body of this rule instantiation has failed (since there are two goals in the example, either one of goals can be chosen e.g., the first goal, $g_0^0(n,w)$, is failed). The first player then claims that the tuple corresponding to this goal exists (following a chain $\neg \rel{Train}(n,w)$, $\rel{Train}(n,w)$, and $r_{Train}(n,w)$). The game ends in the node $r_{Train}(n,w)$ (these special types of rule nodes represent tuples in the database) with the opposing player having lost. Thus, the first player has proven that $\rel{Q}(n,s)$ is in the query result.
%\end{Example}
%\subsection{Constructing Provenance Games}
%\label{sec:constr-prov-games}

\subsection{Evaluation Games}
\label{sec:eval-game}

Given a query $Q$ and \emph{EDB} database instance $I$, a provenance game is constructed by creating a positive and negated tuple node $\rel{R}(c_1, \ldots, c_n)$ for each n-ary predicate $\rel{R}$ and for all combinations of constants $c_i$ from $\adom{I}$. 
Similarly, nodes are created for grounded rules, i.e., versions of a rule where variables have been replaced with constants from the database, and each goal in the body of a rule. For instance, $\rel{Q}(n,s) \dlImp \rel{Train}(n,w),\rel{Train}(w,s)$ is a grounded version of rule $r_0$ in Fig.~\ref{fig:running-example-db}. 
In the game, such rule groundings are labelled $r(\vec{c})$ for a rule $r$ and variables of the rule bound to a vector of constants $\vec{c}$. Finally, \emph{EDB} rule nodes are added for each tuple in $I$, e.g., $r_{Train}(n,w)$ for the tuple $(n,w)$. Tuple nodes are connected to the grounded rule nodes that derive them (have the tuple in their head), rule nodes to goal nodes for the grounded goals in their body (goals  are labelled with their position in the body e.g., $g_0^0$ is the first goal of rule $r_0$), and goal nodes to negated tuple nodes corresponding to the goal (positive goals) or positive tuple nodes (negated goals). Intuitively, such a game encodes which rule groundings would derive a tuple and what input tuples are needed (or required to be absent) to make a rule grounding succeed. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{Definition}[Evaluation Game]
  \label{def:evaluation-game}
  The evaluation game $G_{Q,\D}$ for a program $Q$ and EDB instance $\D$ is a game graph defined over the grounded program. The nodes of $G_{Q,\D}$ are:
  \begin{itemize}
  \item A postive and a negative relation node $R(x)$ and $\dlNeg R(x)$ for each ground atom $R(x)$
  \item A rule node $r_i(x,y)$ and corresponding goal nodes $g_i^j(x_j)$ or $g_i^j(x_j, y_j)$ for each grounded rule $r_i$. Here, $x_j$ and $y_j$ denotes the arguments of the $j^{th}$ goal in the grounded rule.
  \item An EDB rule node $r_R(x)$ for every tuple $R(x) \in \D$.
  \end{itemize}
%The edges of $G_{Q,\D}$ are: \textcolor{blue}{$(\dlNeg R(x), R(x))$} for each relation node pair $R(x)$ and $\dlNeg R(x)$;
%\textcolor{blue}{$(R(x),r_i(x,y))$} for each relation node $R(x)$ and rule node $r_i(x,y)$ where the grounded head of grounded rule $r_i(x,y)$ is $R(x)$; 
%\textcolor{blue}{$(r_i(x,y),g_i^j(x_j))$} for each rule node $r_i(x,y)$ and corresponding goal node $g_i^j(x_j)$; 
%\textcolor{blue}{$(g_i^j(x_j), \dlNeg R(x))$} for each node for a negative goal $g_i^j$ where $R$ is the goal's predicate;
%\textcolor{blue}{$(g_i^j(x_j),R(x))$} for each node for a positive goal $g_i^j$ where $R$ is the goal's predicate; 
%\textcolor{blue}{$(R(x),r_R(x))$} for each relation node $R(x)$ and rule node $r_R(x)$ if $R(x) \in \D$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Solved Games}
\label{sec:solved-game}

Once a game graph is constructed, it can be solved through a fix point computation: initially only nodes without outgoing edges are lost; if a node has an edge to a lost node, then this node is won (the player has a winning strategy by moving to the lost node); if all outgoing edges of a node lead to a won node, then the node is lost (no matter which move the player takes, he will loose). Note that it is possible to compute this fix point by evaluating a datalog rule 
%\begin{align*}
$\rel{win}(X) \dlImp \rel{move}(X,Y), \dlNeg \rel{win}(Y)$
%\end{align*}
under the well-founded semantics~\cite{FK97} where $\rel{move}$ is the edge relation of the provenance graph. 
%\subsection{Solved Games}
%\label{sec:solved-game}
When describing the play of the game for $Q$, we have made the assumption that both players are playing perfectly. 
The claim that a tuple 
%$\rel{Q}(\cnst{j})$ 
exists can only be considered proven if the opposing player does not make a mistake (fails to find the correct argument for refuting the claim even if it exists) and should only be considered refuted if the first player plays perfectly (finds a valid proof if it exists). K\"ohler et al.~\cite{KL13}  demonstrated a connection between \emph{winning strategies} in provenance games and query evaluation. A player has a winning strategy in a position if no matter what moves are taken by the opposing player, the player can force a win. A position which permits a winning strategy is \textit{won} while a position with a winning strategy for the opponent is \textit{lost}. A solved game is a game where each position is marked as won or lost. 
Formally, given an evaluation game $G_{Q,I}(V,E)$, we use
$G^{\Gamma}_{Q,I}(V,E,\Gamma)$ to denote the solved game where
$\Gamma: V \to \{\textcolor{DarkGreen}{won},\textcolor{DarkRed}{lost}\}$ is a function that maps nodes to their won/lost
state.  Any relation node that is marked as won corresponds to an existing tuple in
the \emph{IDB} or \emph{EDB} and a lost relation node corresponds to a missing tuple. Thus,
solving the instantiated game for a program $Q$ and instance $I$ is akin to
evaluating $Q$ over $I$.
%For example,  Fig.~\ref{fig:exam-pg-why-NY-seattle} shows a solved game where won positions are green and lost positions are red.  As proven in~\cite{KL13}, a tuple node in a provenance game is won iff the corresponding tuple exists. The same holds for goal nodes. A rule node is lost iff the corresponding rule instantiation is successful (the attempt to refute the rule failed).


%\emph{Provenance Games} as introduced by K\"ohler et al.~\cite{KL13} % are a crude
%% way to
%provide explanations $\explainq(P,Q(t),I)$ for all atoms $Q(t)$ in non-recursive \datalogneg programs $P$.
%%
%%Provenance games express a non-recursive \datalogneg program evaluation 
%They express evaluation as a 2-player game in a game-theoretic sense. The provenance game consists of 1) a \emph{game graph} and 2) a set of simple rules. In the game graph, nodes are positions in the game while directed edges represent potential moves that the player in the originating node can choose from. The game rules are as follows:
%a game starts in any position and players take turns by choosing an outgoing edge to
%follow until the game ends in a node without an outgoing edge. At this point, the player who has to make the next move has \emph{lost}. 
%% In such a game, one an reason over the \emph{won}/\emph{lost} state of nodes based on
%% winning strategies. Each player who has to make the next move plays perfectly
%% (always chooses the best move from the current position). 
%Since each player is assumed to play perfectly, a node is \emph{won} (the player won) if following any outgoing edge reaches a lost node. 
%%if by following any outgoing edges to a lost node, the player can win. 
%% and -> or for now  (2 different cases to lost)
%A node is \emph{lost} if all outgoing edges lead to won nodes (there is no way for this player to win).
%% if the other player plays perfectly.
%As shown in~\cite{KL13}, games for non-recursive \datalogneg programs (FO queries) 
%have no cycles and thus do not allow for draws. 
%%As provenance game graphs for
%%non-recursive \datalogneg programs (FO queries) as introduced by K\"ohler et
%%al.~\cite{KL13} do not have cycles, draw positions do not need to be considered.
%%
%% TODO: explain following paragraph in 'solving games'
%% If a the provenance game graph is modelled as an edge relation 
%% $\rel{move}(X,Y)$, then the won, lost state of nodes in the game can itself be
%% computed by evaluating the following non-stratified Datalog program 
%% $\rel{win}(X) \dlImp \rel{move}(X,Y), \dlNeg \rel{win}(Y)$ under the
%% well-founded semantics~\cite{FK97}. Intuitively, a node is lost if
%% either it has no outgoing edges or if all its outgoing edges lead to won nodes
%% (no matter where the player moves he will loose). A node is won as long as one
%% of its outgoing edges leads to a lost node (the player can move to this node to
%% win). In~\cite{KL13} a connection between the won/lost state of nodes in the
%% game and query evaluation and the irrelevance of bad moves (a move that lets the
%% other player win unnecessarily) for provenance was proven. Here, we omit further
%% details of the game theoretic foundation of provenance games unless it is
%% necessary for understanding the approach.
%% Instead we illustrate how to construct and solve a provenace game graph
%% according to K\"ohler et al.~\cite{KL13}.
%%
%Now, we illustrate how to construct and solve a provenace game graph according to
%K\"ohler et al.~\cite{KL13}.
%
%% First, an \textbf{evaluation game} graph is derived from a Datalog program and a
%% given EDB instance, then solved by determining lost and won position
%% (the \textbf{solved evaluation game}). Based on lost and won positions in a
%% solved game we can determine 1) IDB instances and 2) for each existing IDB
%% tuple (won position) we can determine parts of the graph which are irrelevant
%% for deriving this tuple (corresponding to suboptimal moves in the corresponding
%% game). These suboptimal moves can be identified based on the solved game. If we
%% compute the subgraph induced by edges that are ``good moves'' then we get a
%% \textbf{provenance game} (PG) which only contains ``relevant'' information.
%% Finally, restricting such a game to nodes connected to the nodes matching the
%% user question results in a provenance game for this question (which
%% we also refer to as the explanation of this question). The naive algorithm for
%% computing the provenance game for a question strictly follows these phases.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Evaluation Games}
%\label{sec:overview-gp}
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{figure}[t]
%%   \centering
%% \resizebox{0.12\textwidth}{!}{\mbox{\input{figures/game4.dot.tex}}}
%% \hfill
%% {\footnotesize\begin{tabular}[b]{|@{~}c@{~}|@{~}p{0.55\columnwidth}@{~}|}
%% \hline
%% \textbf{Move} & \textbf{Claim made by making the move}\\
%% \hline
%% \hline
%%   $\mathsf{A}\stackrel{\exists}{\leadsto} \mathsf{R}$ & ``$A$ is true: it's the head of this instance of ${R}$.''\\
%% \hline
%% \hline
%%   $\mathsf{R}\leadsto \mathsf{G}$ & ``Positive goal $g_k ({=}A')$ in your rule body fails!''\\
%% \hline
%%   $\mathsf{G}\leadsto\neg \mathsf{A}$ & ``No! Its negation $\neg A'$
%%   fails and $A'$ is true.''\\
%% \hline
%%  $\neg \mathsf{A}\leadsto \mathsf{A}$ & ``No:  atom $A'$ fails!''\\
%% \hline
%% \hline
%%   $\mathsf{R}\leadsto \mathsf{N}$ & ``Negative goal $\neg A'$ in the rule body fails.''\\
%% \hline
%%   $\mathsf{N}\leadsto \mathsf{A}$ & ``No: $\neg A'$ succeeds, but $A'$ fails.''\\
%% \hline
%% \end{tabular}}
%% %
%% %
%% \caption{\small Move types of the query evaluation game (left) and
%%   implicit claims made (right). Moving along an edge, a player aims to
%%   verify a claim, thereby refuting the opponent. Initially, player \pI
%%   is a verifier, trying to prove $A$, while \pII tries to spoil this
%%   attempt and refute it. Roles are swapped (\pI $\rightleftharpoons$
%%   \pII) when moving through a negated goal ($\mathsf{R}{\leadsto}\mathsf{N}{\leadsto}\mathsf{A}$).}
%%   \label{fig-game-overview}
%% \end{figure}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%% remove First, an 
%\emph{Evaluation game} is constructed from a program and a
%given EDB instance using the following definition.
%% Consider a datalog program $Q$ that is evaluated of an EDB instance $\D$.  Query
%% evaluation of $\Q(\D)$ can be seen as a game between players \pI and \pII who
%% argue whether an atom $A(t) \in \Q(\D)$. The evaluation game graph is composed
%% of three classes of nodes: 
%% % as shown on the left of \Figref{fig-game-overview}:
%% \textit{Relation nodes} (depicted as circles),
%% \textit{Rule nodes} (depicted as rectangles), and
%% \textit{Goal nodes} (rectangles with rounded corners).
%% % \end{itemize}
%% Relation nodes and goal nodes can be positive or negated.
%% % In the following, we summarize the game argumentation structure presented by
%% % K\"ohler et al. using the following example from~\cite{KL13}:
%% % %
%% % %
%% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% % \begin{equation}
%% % %
%% % r_1: \quad \rel{A}(X)  \la  
%% %   \underbrace{\rel{B}(X,Y)}_{\mathnormal{g_1}},\;
%% %   \underbrace{\neg\,\rel{C}(Y)}_{\mathnormal{g_2}} 
%% % %
%% %   \tag{\Pabc}
%% % \end{equation}
%% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%% % Figure~\ref{fig:abcgamediagram} shows the game template (the possible 
%% % argumentation structure) for the Datalog program shown \Pabc above.  
%% %
%% % For example, to explain why $A(X)$ is in the IDB, the player \pI has to prove 
%% % that there is at least one binding of rule $r_1$ that is successful. The other
%% % player (\pII) can try to refute this claim moving to one of the goals, e.g., 
%% % $g_1^1(X,Y)$ which represents that goal $B(X,Y)$, for this rule instantiation 
%% % which he believe fails. Player \pI has to respond by claiming that the negation
%% % of the goal atom fails which player \pII has to respond to by claiming that 
%% % $B(X,Y)$ does not exit. At this point, if in fact $B(X,Y)$ does not exist then 
%% % player \pII wins (has successfully proven that this rule instantiation fails). 
%% % If $B(X,Y)$ is in the EDB instance, then player \pI can move to $r_{B}(X,Y)$ and
%% % player \pII will loose (\pI has falsified \pII's claim that the goal failed).
%% 
%% %%%%%%%%%%%%%%%%%%%%
%% \mypara{Relation nodes} A positive relation node $A(x)$ represents the claim
%% that this atom is part of the instance whereas $\neg A(x)$ represents the claim
%% that the tuple is missing. In the game, a negative relation node is always
%% connected to a positive.
%% % (i.e., if a player claims $A(x)$ then the other player has to respond by
%% % claiming the oposite). 
%% The won/lost state for relation nodes corresponds the truth of the claim, e.g.,
%% a node $\neg A(x)$ is won and $A(x)$ is lost if tuple $A(x)$ is not part of the
%% IDB instance.
%% % The absence of a tuple ($\neg A(x)$) can be proven by demonstrating that all
%% % rules with this atom as a head fail.
%% To disprove the claim $\neg A(x)$ (and, thus, prove $A(x)$), at least one rule
%% with this atom as a head has to fire successful. 
%% % Thus, a node $\neg A(x)$ will always be connected to all rule nodes (rule 
%% % instantiations) with head $A(x)$. 
%% %
%% % TODO: Add example
%% %
%% % For example, for some $A(x)$, there may be many binding of rule $r_1$ (one
%% % for any possible value of $y$).
%% % \footnote{In provenance games, possible values are restricted to the
%% %           active domain of the EDB instance, i.e., $\adom{I}$.}
%% 
%% %%%%%%%%%%%%%%%%%%%%
%% \mypara{Rule and goal nodes} Rule nodes correspond to rule instantiations. A
%% rule node $r(\vec{c})$ stands for the assignment of the constants from the list
%% $\vec{c}$ to the variables of $r$. Variables are ordered according to their first
%% occurrence in the rule (including occurrences in the head).
%% %provide the constants in this order.
%% A rule node is connected to the positive relation node for the
%% head predicate of the rule with the restriction of $\vec{c}$ to the head 
%% variables as arguments. 
%% % A rule node is lost if the rule instantiation is
%% % successful, i.e., attempts to refute the rule body will fail, and won otherwise.
%% Note that a provenance game also contains (lost) rule nodes to
%% represent EDB facts (the tuples in the database instance).
%% Furthermore, a rule node is connected to goal nodes representing all the 
%% instantiated goals. We label goals by their position and the rule they belong
%% to. For example, $g_2^1$ would be the first goal of rule $r_2$.
%% %
%% % %%%%%%%%%%%%%%%%%%%%
%% % \mypara{Goal nodes}
%% A goal node is connected 
%% % to the corresponding rule node and %% to a relation node representing the goal's predicate but opposite claim, i.e., a 
%% negated relation nodes for positive goals and positive relation nodes for
%% negated goals).
%% A goal node is won if it is connected to a failed rule node (successful rule
%% instantiation) and a failed relation node (representing the opposite claim).
%% 
%% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% % \begin{figure}[t]
%% %   \centering
%% %   \mbox{\resizebox{.95\columnwidth}{!}{\input{figures/abc-graph-no-color.dot.tex}}}
%% %   \caption{Game $G_\PabcD$ for $\D= \{ B(a,b), B(b,a), C(a)\}$}
%% %   \label{fig:gamegraphpabc}
%% % \end{figure}
%% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%% % To fully instantiated a game $G_{Q,\D}$ for a program $Q$ and instance $\D$
%% % which encodes the evaluation of a program $Q$ over edb instance $\D$ the game
%% % graph is created using the following schema:
%% %
%% % We will briefly explain in Section~\ref{sec:top-down-datalog-comp} how to
%% % instantiate such a game using a Datalog program.
%% % In Section~\ref{sec:solved-games} we will explain how actual rule instantiations
%% % and facts are determined by solving the game.
%% %
%% % In \figref{fig-reduction-ex}, we show Datalog rules that
%% % define the move relation $\mathtt{M}$ of the instantiated game $G_{\Pabc,\D}$ for program \Pabc with instance $\D$.
%% % Here, $\Domain$ is a relation that contains the active domain of \Pabc and $D$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{Definition}[Evaluation Game]
%  \label{def:evaluation-game}
%  The evaluation game $G_{Q,\D}$ for a program $Q$ and EDB instance $\D$ is a game graph defined over the grounded program. The nodes of $G_{Q,\D}$ are:
%  \begin{itemize}
%  \item A postive and a negative relation node $R(x)$ and $\dlNeg R(x)$ for each ground atom $R(x)$
%  \item A rule node $r_i(x,y)$ and corresponding goal nodes $g_i^j(x_j)$ or $g_i^j(x_j, y_j)$ for each grounded rule $r_i$. Here, $x_j$ and $y_j$ denotes the arguments of the $j^{th}$ goal in the grounded rule.
%  \item An EDB rule node $r_R(x)$ for every tuple $R(x) \in \D$.
%  \end{itemize}
%The edges of $G_{Q,\D}$ are: \textcolor{blue}{$(\dlNeg R(x), R(x))$} for each relation node pair $R(x)$ and $\dlNeg R(x)$;
%\textcolor{blue}{$(R(x),r_i(x,y))$} for each relation node $R(x)$ and rule node $r_i(x,y)$ where the grounded head of grounded rule $r_i(x,y)$ is $R(x)$; 
%\textcolor{blue}{$(r_i(x,y),g_i^j(x_j))$} for each rule node $r_i(x,y)$ and corresponding goal node $g_i^j(x_j)$; 
%\textcolor{blue}{$(g_i^j(x_j), \dlNeg R(x))$} for each node for a negative goal $g_i^j$ where $R$ is the goal's predicate;
%\textcolor{blue}{$(g_i^j(x_j),R(x))$} for each node for a positive goal $g_i^j$ where $R$ is the goal's predicate; 
%\textcolor{blue}{$(R(x),r_R(x))$} for each relation node $R(x)$ and rule node $r_R(x)$ if $R(x) \in \D$.
%% \end{itemize}
%\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%% Furthermore, we create a \emph{rule node} for each rule $r_i$ in the ground program 
%% with a unique identifier $f_{r_i}(X_1,\dots,X_n)$ including the rule number and 
%% the assignments of variables found in the rule's body to constants.  There is
%% an edge from the ground head atom to the ground rule node (cf.
%% \figref{fig-reduction-ex} first line of middle block).
%% For example, the skolem function $f_{r_1}(a,b)$ encodes the whole rule body $r1:[B(a,b),\neg{}C(b)]$.
%
%% %
%% Then, we add moves from rule node $r_i$ to its \emph{goal nodes} $g_i^j$. 
%% Goal nodes are identified by the rule number $i$ they occur in, their
%% positions $j$ within the body, and the bound constants. (cf. lines 2 and 3 of
%% middle block). From positive (negative) goal nodes, we move to negative (positive) relation
%% nodes keeping the bound constants fixed (cf. lines 4 and 5 of middle block).
%% %
%% Finally, for \edb relations, we add an edge from the positive relation node
%% $R(\bar c)$ to a rule node $\mskol{r_R}{\bar c}$ iff $R(\bar c) \in D$. This
%% ensures that a player reaching the relation node $R(\bar c)$ wins iff $R(\bar c)
%% \in D$.
%%
%Fig.~\ref{fig:solved-game-example} shows the instantiated game for
%query \Pabc with input database $\D= \{B(a,b), B(b,a), C(a)\}$:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{equation}
%%
%r_1: \quad \rel{A}(X)  \la  
%  \underbrace{\rel{B}(X,Y)}_{\mathnormal{g_1}},\;
%  \underbrace{\neg\,\rel{C}(Y)}_{\mathnormal{g_2}} 
%%
%  \tag{\Pabc}
%\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%.
%
%% Usually, an evaluation game starts with I claiming that a ground atom
%% $A(x)$ is true. That is she starts the game in a relation node for $A$ corresponding to a concrete binding of variables to $x$. 
%% To substantiate her 
%% claim she moves to a rule that has $A$ as a head atom and specifies
%% constants for the remaining
%% existentially quantified variables in the body of the rule. Now, II tries to reject
%% the validity of the rule by selecting a goal atom (\eg $B$) in its body that he thinks is not
%% satisfied (\eg II moves to the goal node for $B$).
%% %
%% %
%% \pI then moves to a negated relation node for this goal
%% (eg, a node $\neg B$), claiming the goal is
%% true because its negation is false. From here, \pII moves to the relation node
%% $B$, questioning \pI's claim that $B$ is true. The game then
%% continues in the same way. Note that the graph on the left of in \figref{fig-game-overview} is a schema-level
%% description. When one cycle
%% (relation$\leadsto$rule$\leadsto$goal$\leadsto$$\neg$relation$\leadsto$relation) is complete, the actual fact that 
%% is argued about has changed (\eg from $A$ to $B$). If \pII selects a negated goal (\eg $\neg C$) in the body of a rule then player \pI moves directly
%% from the negated goal node to the relation node for $C$. This essentially switches the roles of I
%% and \pII since now player \pII has to argue for a relation node $C$.
%
%% We now demonstrate the general argumentation scheme for a concrete \datalogneg
%% program \Pabc. The program $\Pabc$ consists of a single rule $r_1$: 
%
%%
%%
%%
%% The game diagram for \Pabc is shown in \figref{abcgamediagram}. Player \pI
%% starts in a relation node of type $A(X)$ with a concrete instatiation $X=x$ 
%% to prove that $\rel A(x)\in\Q(\D)$. 
%% In her first move, she picks the rule $r_1$ together with
%% bindings for all existentially quantified variables in $r_1$, 
%% which is just a instatiation $y$  for $Y$ in $r_1$; 
%% essentially
%% picking a ground instance $r_1(x,y)$ such that the variable $X$ is bound to the
%% desired $x$. She claims the rule body is satisfied.
%%
%%
%%
%% If this is not the case, \pII can falsify the claim by
%% selecting a \emph{goal} from the body, i.e., either $g_1^1(x,y)$, %
%% thus making a counter-claim that $\rel B(x,y)$ is false, or %
%% %
%% $g_1^2(y)$, claiming instead that $C(y)$ is true. \textit{Positive case,} \eg
%% \pII moved to $g_1^1(x,y)$.  Player \pI
%% will move from $g_1^1(x,y)$ to $\neg B(x,y)$, from which \pII will move to
%% $B(x,y)$. In this node, there is an edge for player \pI if and only if $B(x,y)
%% \in D$, that is if there is a trivial, bodyless rule $r_B(x,y)$ representing
%% this fact. Thus, \pI wins the game if $B(x,y) \in D$ and \pII wins if $B(x,y)
%% \not\in D$. \textit{Negative case,} \eg \pII just moved to $g_1^2(y)$. Player
%% \pI moves to the instatiation $\mathtt{C}(y)$ of relation node $C(X)$. 
%% For this move in the diagram, variables used in the goal node are explicitely 
%% renamed to the single variable name used in the corresponding relation node.
%% With this move, \pII loses and \pI wins if $C(y) \not\in D$;
%% \pII wins the argument if $C(y) \in D$ by moving to the trivial rule node,
%% forcing \pI to lose.
%
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \subsection{Game Templates}
%% \label{sec:game-temp}
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{figure}[t]
%%   \centering
%%    \mbox{\resizebox{0.62\columnwidth}{!}{\input{figures/abc-template.dot.tex}}}
%%   \caption{Example Game Template}
%%   \label{fig:abcgamediagram}
%% \end{figure}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%% We now define the game templates for a given Datalog$^{\neg}$ program $Q$. 
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{Definition}[Game Template]
%% Let $\Q$ be a Datalog$^{\neg}$ program. The game template $\gametemplate{Q}$ is a node and edge-labelled graph constructed as follows:
%% \begin{itemize}
%% \item For each edb relation $R$ we add a rule node $r_{R}(\vec{X}_R)$ were $\vec{X}_R$ are fresh variables - one per attribute of $R$. Also add a negated relation node $\neg R(\vec{X}_R)$ and positive relation node $R(\vec{X}_R)$. Connect $r_{R}$ to $\neg R$ and $\neg R$ to $R$.
%% \item For each idb relation $R$ we add positive and negative relation nodes. The negative relation node is connected to the positive one. Furthermore, we connect the positive one to all rules have $R$ as their head atom. The edbe between the relation node $R$ and a the node for such a rule $r_i$ is labelled $\exists \vec{X}_{Body(r_i)}$ where $Body(r_i)$ are the variables which only occur in the body of $r_i$.
%% \item For each rule $r_i$ in $Q$ add a node $r_i(\vec{X}_i)$ where $\vec{X}_i$ are the variables occurring in $r_i$.
%% \item For each goal $g_i^j$ of a rule $r_i$ add a node $g_i^j(\vec{X}_{i,j})$ where $\vec{X}_{i,j}$ are all variables occurring in $g_i^j$. Add an edge from $r_i$ to $g_i^j$. Let $R_{i,j}$ denote the relation accessed by goal $g_{i,j}$. If the goal is positive we connect $g_{i,j}$ to $\neg R_{i,j}$. Otherwise, $g_{i,j}$ is connected to $R_{i,j}$. In both cases, the edge is labelled $\vec{X} := \vec{X}_{i,j}$ where $\vec{X}$ are the variables of the relation node.
%% \end{itemize}
%% \BG{Replace Body(r) if we end up introducing a different notation in the datalog background section}
%% \end{Definition}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%% As the name suggests, a game template for $Q$ defines the types of nodes and game moves that will appear in the instantiated a game for $\Q$ and a given \edb instance $\D$. 
%% For instance, consider $\gametemplate{\Pabc}$, the game template for our example program $\Pabc$. There are two relations $\rel{B}$ and $\rel{C}$ in the edb. Thus, the game template has the corresponding rule, positive relation, and negative relation nodes. The program consists of one rule with a positive and a negated subgoal. The positive is connected to the negated relation node for $\rel{B}$ and the positive relation node for $\rel{C}$. Note that because we connected nodes in this way, a positive goal node will be won if the corresponding tuple exists and will be lost if the tuple does not exist. The oposite is true for negative goal nodes. 
% 
%
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \subsection{Instantiated Games}
%% \label{sec:inst-games}
%
%
%% The game template for a program defines what types of moves will be possible in a concrete instantiation of such a template. 
%
%
%
%%
%
%% \mypara{Acyclicity of FO Games}
%% For FO queries, represented by non-recursive \datalogneg programs,
%% no relation node is reachable from itself and the resulting game graph is acyclic.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Solved Evaluation Games}
%\label{sec:solved-games}
%
%An evaluation game graph, modelled as an edge relation $\rel{move}(X,Y)$, 
%can be solved by evaluating the non-stratified Datalog program 
%$\rel{win}(X) \dlImp \rel{move}(X,Y), \dlNeg \rel{win}(Y)$ under the
%well-founded semantics~\cite{FK97}.
%In the \emph{solved game}, every node is marked as either won or lost.
%% \footnote{As mentioned before, there may also exist
%%   draw positions in a game, but it has been shown that the solved instantiated
%%   game for non-recursive datalog queries contains only won and lost positions.}
%Formally, given an evaluation game $G_{Q,I}(V,E)$, we use
%$G^{\Gamma}_{Q,I}(V,E,\Gamma)$ to denote the solved game where
%$\Gamma: V \to \{\textcolor{DarkGreen}{won},\textcolor{DarkRed}{lost}\}$ is a function that maps nodes to their won/lost
%state.  Any relation node that is marked as won corresponds to an existing tuple in
%the IDB or EDB and a lost relation node corresponds to a missing tuple. Thus,
%solving the instantiated game for a program $Q$ and instance $I$ is akin to
%evaluating $Q$ over $I$.  The solved game for the running example in this
%section is also shown in \figref{fig:solved-game-example}. Here, we see that \emph{I} has
%a winning strategy for e.g., $A(a)$, $B(b,a)$, and $C(a)$, as these are part of instance.
%
%%That is these tuples are part of the instance.  
%% It has been proven in~\cite{KL13} that solved evaluation games are draw-free
%% for non-recursive Datalog programs and the won and lost labels of relation 
%% nodes correspond to the existence (respective absence) of atoms in the IDB/EDB.
%% % Here we restate the relevant part of that theorem.
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{Theorem}[Instantiated Games Encode Query Evaluation]
%%   Consider a 
%%   non-recursive \datalogneg program $\Q$ with output relation
%%   %
%%   %
%%   %
%%   \rel{R_{ans}} evaluated over edb instance $\D$. 
%%   Let  $\solved{G_{\Q,\D}} = (V,M,\gamma)$ be the
%%   solved instantiated game for $\Q$. Then:
%
%%   \begin{center}
%%     \begin{math}
%%       \Q(\, \rel{R_{ans}}(\bar x)\, ) = \left\{
%%         \begin{array}{@{}c@{}}
%%           \true{}\\
%%           \false{}\\
%%         \end{array} \right\}
%%       \Leftrightarrow
%%       \gamma(\, \mskol{ans}{\bar x} \,) =
%%       \left\{
%%         \begin{array}{@{}c@{}}
%%           \wonPos{\won}\\
%%           \lostPos{\lost}\\
%%         \end{array} \right\} 
%%     \end{math}
%%   \end{center}
%% \end{Theorem}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{proof}
%%   See~\cite{KL13} for a proof sketch.
%% \end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Solved Evaluation Games Without Bad Moves aka Provenance Games}
\subsection{Deleting Bad Moves aka Provenance Games}
\label{sec:provenance-cond-solved-game}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[t]
%  \centering
%  { \mbox{\resizebox{.95\columnwidth}{!}{\input{figures/abc-graph.dot.tex}}}
%  }
%\caption{Solved instantiated game $\gsol_\PabcD$. %
%    Lost positions are (dark) red; won positions are (light) green.  Provenance
%    edges (good moves) are solid; bad moves are dashed.  $A(a)$ (resp.\ $A(b)$)
%    is true (resp.\ false), indicated by position value \won (resp.\ \lost).
%    The game provenance $\gprov(A(a))$ explains why $A(a)$ is true.
%    % $\gprov(A(b))$ explains why-not $A(b)$.
%  }
%  \label{fig:solved-game-example}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A solved game already provides all information about the provenance
of program $Q$. However, parts of the game graph are irrelevant for explaining
existing and missing tuples in the IDB relations. Intuitively, if we look at
the subgraph rooted at an (negated) IDB relation node, this subgraph
explains how the tuple was produced (or failed to be produced). 
% From the game theoretic point of view, 
Some edges in such a subgraph correspond to non-optimal moves while we require
players to play optimal. We use an edge-labeling function  $\lambda: V\times V \to \{ \textcolor{DarkGreen}{good}, \textcolor{DarkRed}{bad}\}$ to distinguish
different types of moves. $\lambda(x_1,x_2) = \textcolor{DarkRed}{bad}$ if both $x_1$ and $x_2$ are won, otherwise $\lambda(x_1,x_2) = \textcolor{DarkGreen}{good}$.
% For example, it does not make sense to move from a won position to a won
% position because this would result in a win for the opposing player (if that
% player plays correctly).
% There is a beautiful correspondence between these bad
% moves, irrelevant parts of the provenance, and ``bad'' resolution steps, i.e.,
% resolution steps that do not help us provide evidence for an IDB fact. 
% For example, moving from a won IDB tuple node $t$ to a won rule node $r$ can be
% interpreted as trying to prove that $t$ can be derived through instantiating
% rule $r$ according to that rule node. However, this resolution is not
% successful, because $r$ is won (for the other player).  In general, we can
% identify bad moves in the solved game and determine the subgraph induced by the
% set of edges corresponding to good moves. We call the result of this step a
% \textbf{provenance game} and use $\gprov(x)$ to denote the provenance game
% restricted to nodes connected to node $x$.
% 
% First, only nodes \emph{reachable} from $x$ can influence the outcome at $x$,
% i.e., only nodes and edges in the transitive closure $\Flr^+(x)$.  Thus, one
% expects $\gprov(x)$ to depend only on $\Flr^+(x)$. In fact two results
% from~\cite{KL13} provide a solid foundation for this claim, because 1)
% provenance games model query evaluation and 2) in games only nodes reachable
% from a node $x$ can influence that nodes won/lost state. That is, only nodes
% connected to $x$ should be considered to be in the provenance of $x$, because
% the won/lost state of all remaining nodes cannot possibly influence the won/lost
% state of $x$. In addition, one expects the value $\gprov(x)$ of position $x$ to
% be independent of ``bad moves'', i.e., which give the opponent a better outcome
% than necessary. Again, the justification to exclude this moves is based on the
% game theoretic foundation of provenance games. A bad move (from a won to a won
% node) can never be part of a winning strategy, i.e., it represents an attempt to
% prove a fact that fails. For example, for an existing IDB instance tuple $Q(t)$
% (won node) there has to exist at least one successful rule instantiation.  There
% may be arbitrarily many failed rule instantiations. However, these failed ways
% of deriving $Q(t)$ are irrelevant for explaining existence of $Q(t)$ as long as
% there is one successful derivation.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Edge Labels]
%   Let $\gsol=(V,M,\gamma)$ be a solved game.  The edge-labeling
%   $\lambda: V\times V \to \{ good, bad\}$ defines a color
%   for a subset of edges from $M$ as follows:
%   \begin{align*}
%     \lambda((x_1,x_2)) =
%     \begin{cases}
%       bad & \text{if}\; win(x_1) \wedge win(x_2)\\
%       good & \text{else}
%     \end{cases}
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In \figref{fig-prov-edges} we use $\gamma(x)$ and $\gamma(y)$, i.e.,
% node labels \won, \drawn, and \lost of moves $(x,y)\in M$ to derive an
% appropriate edge label.  This allows us to distinguish
% provenance-relevant (``good'') moves (\emph{winning}, \emph{drawing},
% or \emph{delaying}), from irrelevant (\emph{bad}) moves.
The \emph{provenance game} is derived from a solved game by excluding bad moves.
The game provenance for a particular tuple (relation node) is defined as the node's
transitive closure, i.e., for a question $\rel{Q}(t)$, 
the subgraph rooted at the nodes matching question
(in case $t$ only has constants, this will be exactly one node). For $\whyq$ 
($\whynotq$) questions, only subgraphs rooted at won (lost) nodes 
are considered.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Provenance Game] Let $\gsol=(V,M,\glabel)$ be a solved
  game. The \emph{provenance game} $\gprov$ is the
  $\textcolor{DarkGreen}{good}$-labeled subgraph of \gsol. For $x\in V$, we define $\gprov(x)$ as
  the subgraph of \gprov, reachable via $\lambda$ edges. Note that for a user
  question $\rel{Q}(t)$, $\gprov(\rel{Q}(t))$ is the explanation for $\rel{Q}(t)$ according to Definition~\ref{def:explanation}.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For example,  Fig.~\ref{fig:exam-pg-why-NY-seattle} shows a provenance game where won positions are green and lost positions are red.  As proven in~\cite{KL13}, a tuple node in a provenance game is won iff the corresponding tuple exists. The same holds for goal nodes. A rule node is lost iff the corresponding rule instantiation is successful (the attempt to refute the rule failed).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Example}
%   Consider the solved game for the example query $\Pabc$ as shown in Figure
%   \figref{fig:solved-game-example}. Bad moves are shown as grey edges. For
%   instance, $\rel{A}(a)$ is justified by the successful rule derivation
%   $r_1(a,b)$, whereas the edge between $\rel{A}(a)$ and the potential rule 
%   derivation $r_1(a,a)$ is not part of the provenance, because this rule
%   derivation has failed.
% \end{Example}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Naive Provenance Game Computation}
%\label{sec:top-down-datalog-comp}
%
%Having presented some basic background on provenance games, we are now ready to
%explain the top-down approach for computing a provenance game that was
%introduced in~\cite{KL13}. A Datalog program is generated that
%computes the move graph of the instantiated game according to Definition~\ref{def:evaluation-game}.
%Fig.~\ref{fig-reduction-ex} shows the result for the example program $\Pabc$.  % with an active domain of $\adom{I} = \{a,b\}$.
%Here, domain $\Domain$ denotes a relation storing $\adom{I}$, and skolem functions are used to create node identifiers.
%% We use Skolem functions to create ``node identifiers''. E.g., for a ground atom
%% $\mathtt{S(a_1,\dots,a_n)}$ we use $f_S(\mathtt{a_1,\dots,a_n})$ for its positive relation nodes and 
%% $f_{\neg{}S}(\mathtt{a_1,\dots,a_n})$ for its negative relation node. The first three
%% rules in \figref{fig-reduction-ex} create an edge from the negative to the
%% positive node.\footnote{The use of Skolems is for convenience only.
%% We could instead use constants and increase the arity of relations accordingly, 
%% or even avoid constants \cite{FK97,flum-TCS-00}.}
%%
%% These rules create EDB rule nodes for every existing tuple in the EDB and
%% connect them to positive relation nodes. Positive and negative relation nodes
%% are created for all possible assignments of variables to values from the active
%% domain. The same applies for rule and goal nodes. These nodes are connected
%% based on assignments of variables to the same constants and the argumentation
%% rules introduce in Section~\ref{sec:overview-gp}, e.g., a relation node for the
%% head predicate of a rule is connected to that rule node. For instance, in the
%% example program $\Pabc$ for an EDB instance with active domain
%% $\adom{I} = \{a,b\}$, a relation node $A(a)$ would be connected to rule nodes
%% $r_1(a,a)$ and $r_1(a,b)$ (variable $X$ is assigned $a$). 
%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}
%  \centering
%%
% {
%    \parbox[b][][t]{.5\textwidth}{
%    \begin{displaymath} 
%      \arraycolsep=1.5pt
%      \begin{array}{lcl}
%        \textnormal{\textbf{Atoms} $A$,$B$, \textbf{and} $C$} \\
%        \mrel{M}(\mskol{\neg{}A}{X}, \mskol{A}{X}) &\la& \Domain(X).\\
%        \mrel{M}(\mskol{\neg{}B}{X,Y},\mskol{B}{X,Y}) &\la&  \Domain(X),\Domain(Y). \\
%        \mrel{M}(\mskol{\neg{}C}{X},\mskol{C}{X}) &\la& \Domain(X). \\[2mm]
%
%        \textnormal{\textbf{IDB} $A$ \textbf{via rule} $r_1$} \\
%        %
%        \mrel{M}(\mskol{A}{X},\mskol{r_1}{X,Y}) &\la& \Domain(X), \Domain(Y).\\
%        \mrel{M}(\mskol{r_1}{X,Y}, \mskol{g_1^1}{X,Y}) &\la& \Domain(X), \Domain(Y).\\
%        \mrel{M}(\mskol{r_1}{X,Y}, \mskol{g_1^2}{Y}) &\la&\Domain(X), \Domain(Y).\\
%        \mrel{M}(\mskol{g_1^1}{X,Y} ,\mskol{\neg{}B}{X,Y}) &\la& \Domain(X), \Domain(Y).\\
%        \mrel{M}(\mskol{g_1^2}{X},\mskol{C}{X}) &\la& \Domain(X).\\[2mm]
%        \textnormal{\textbf{EDB} $B$ \textbf{and} $C$} \\
%        %
%        \mrel{M}(\mskol{B}{X,Y},\mskol{r_B}{X,Y}) &\la& \mathtt{B}(X,Y).\\ 
%        \mrel{M}(\mskol{C}{X},\mskol{r_C}X) &\la& \mathtt{C}(X).
%        \end{array}
%      \end{displaymath}
%    }
%
%  }
%  %
%\caption{Datalog Rules for Computing a Relational Encoding of an Instantiated Evaluation Game for $\Pabc$.}
%\label{fig-reduction-ex}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%The game instantiated in this fashion is then solved by evaluating it together
%with the win-move program using well-founded semantics.
%The provenance game is obtained by discarding bad edges, $\lambda(X,Y) = \textcolor{DarkRed}{bad}$,
%and computing a restricted move relation $M'$ using the following Datalog rule:
%%
%\begin{align*}
%\rel{M'}(X,Y) &\dlImp \rel{M}(X,Y), \dlNeg \rel{win}(X)\\
%\rel{M'}(X,Y) &\dlImp \rel{M}(X,Y), \dlNeg \rel{win}(Y)
%\end{align*}
%%
%These rules ensure that at least one node of each edge is lost.
%To obtain the provenance for a question, the graph needs
%to be restricted to nodes reachable from any node matching the question.
%A Datalog program is generated that computes a reduced
%move relation $\rel{M_u}$ for the why question $\rel{Q}(t)$:
%%
%\begin{align*}
%\rel{M_u}(\mskol{Q}{t},Y) &\dlImp \rel{M'}(\mskol{Q}{t},Y), \rel{Q}(t)\\
%\rel{M_u}(Y,Z) &\dlImp \rel{M_u}(X,Y), \rel{M'}(Y,Z)
%\end{align*}
%%
%Note that in~\cite{KL13}, the last two steps (computing $M'$ and $M_u$)
%are not described in an algorithmically. We have chosen a straightforward 
%implementation. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% probably overlap with intro?
%While this way of computing the game provenance is simple, it is excessively 
%expensive. Already the first step creates an evaluation game graph that is
%exponential in the maximal arity (number of variables) of rules, i.e., 
%${\cal O}(\card{\adom{I}}^{n})$ where $n$ is the maximal arity (number of variables)
%of any rule in the program. For most use cases, $n$ will be in the order of 5 
%to 20. 
%However, even for a small database with 1000 values in the active domain
%and rules with up to 5 variable, this will result in a game with $\sim 10^{15}$ nodes.

%\BG{
%$${\cal O}(\card{\adom{I}}^{n})$$ 
%
%where
%
% $$n = \max_{r \in P}(\card{\varsOf{r}})$$
%
%\mypara{Proof sketch}: The number of edges in the provenance game grow ${\cal O}(\card{\adom{I}}^{n})$, because for a rule with arity $n$ and one of its goals 
%}
%
% \begin{itemize}
% \item Construct game template
% \item Compute top-down instantiation based on domain values (e.g., Figure~\ref{fig-reduction-ex})
% \item leads to the whole game provenance be produced even if only small part needed
% \item because of negation will always be at least size of domain to the power of maximal arity of idb/edb relations large
% \item hard to optimize because we need to come up with values for existential variables
% \item Complexity: 
%   \begin{itemize}
%   \item Create game template is linear in program size (if done right)
%   \item Instantiate game, linear in number of nodes created. How many nodes do we have. Bound by  ${\cal O}(maxArity \times \card{\adom{I}})$ where $maxArity$ is the maximal arity (number of vars) of any rule in program.
%   \end{itemize}
%\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%% Local Variables: 
%% mode: latex
%% TeX-master: "2016_GameProM"
%% End: 


==> overview.tex <==
\section{Overview and Contributions}
\label{sec:contribution}

The existing approach for computing provenance games~\cite{KL13} allows for uniform treatment of provenance and missing answer
problems and provides a meaningful semantics for negation. 
% However, it is prohibitively expensive.
The approach requires instantiation of the whole game for the instance, 
evaluation of a non-stratified Datalog program using well-founded semantics~\cite{FK97} over
this graph, removal of edges that are irrelevant to explain query evalution, and finally determining
%that correspond to bad moves in the game, i.e., moving to a won position by the other player, and, finally, determining
subgraphs related to the user's $\provQ$. %question.
%While this approach is correct, it is prohibitively expensive 
While this approach is correct and easy to understand, it is computationally expensive since it instantiates the whole provenance game. 
% as mentioned in Section~\ref{sec:intro}. %Example\,\ref{ex:example1}.
% its performance is far from optimal.
%A critical problem is the size of the instantiated game which is
%${\cal O}(\card{\adom{I}}^k)$ where $k$ is the maximal number of variables of rules in the input program and $\adom{I}$ is the active domain of the database instance $I$.
%As an example, consider a database with 100 values and a rule with 5 variables.
%There are in the order of $100^5 (= 10^{10})$ nodes in the instantiated game.
Typically, most of the nodes in the instantiated game will not end up being part of the explanation  for the $\provQ$. %provenance question 
%because they are not connected in the
%final provenance graph.
% TODO: 'bad moves' not introduced
%(e.g., they are only reachable through bad moves or are completely disconnected).
To efficiently compute the explanation $\explainq(Q,Q(t),I)$ for a PQ (i.e., $Q(t)$), 
we generate a Datalog program $\GPProg(Q,Q(t),I)$ that computes the part of 
$\provGraph(Q,I)$ %the provenance graph 
for $Q$ belonging to the explanation bottom-up.
Evaluating this program over instance $I$ 
returns the edge relation of $\explainq(Q,Q(t),I)$.
Furthermore, we also support returning provenance games or provenance graphs which encode semiring annotations (e.g., Minimal Why-provenance~\cite{cheney2009provenance}) as explanations. 

% In particular, 


% for a given query $Q$, i.e., relevant parts of the provenance graph for $Q$.


% $\explainq_{\provType}(Q,Q(t),I)$


% Given a question $Q(t)$ 
% for an instance $I$, a query $Q$, and 
% the desired type $\provType$ of provenance graph, 


% we produce a Datalog program $\GPProg_{\provType}(Q,Q(t),I)$. %constructed which 
% Evaluating this program over instance $I$ 
% returns the edge relation of $\explainq_{\provType}(Q,Q(t),I)$, the subgraph of $\provGraph(Q,I)$ %the provenance graph 
% of type $\provType$
% for $Q$ and $I$ 
% (note that we have used $\explainq_{\provType}$ to denote the notion of explanations extended to different provenance graph types).
% restricted to nodes connected to nodes matching the question $Q(t)$ 

%we avoid to generate disconnected nodes that are created in the provenance games 
%based on $t$ in the $\provQ$ %provenance question 
%and the firing rules generated 
%which allow to compute explanations only for the user's $\provQ$.
%In our approach, we employ several optimizations that reduce the amount of
%disconnected nodes that are created.
%First, 
%Our solution exploits information encoded in the $\provQ$, %provenance question $Q(t)$, 
%e.g., based on the constants in $t$, 
%and thus only certain nodes can be connected to $\provQ$ node %$Q(t)$ 
%in the provenance graph. %game.
%For instance, in the running example, $\rel{Q}(n,s)$ can only be
%connected to derivations %instantiations 
%of rule $r_1$ with $X = n$ and $Y = s$.
%In turn, this implies that we are only interested in existence or absence of train tuples
%$\rel{T}(n,Z)$, $\rel{T}(Z,s)$, and $\rel{T}(n,s)$.
%Our approach propagates 
%This type of information is propagated in a top-down traversal of the program, 
%but computes in a bottom-up fashion. 
%with firing rules %generated 
%that capture variable bindings of successful and failed rule derivations %instantiations 
%which guarantee to be in the provenance respective missing answers. 
%(we also check the results of firing rules to ensure that are connected to $Q(t)$).

A main driver of our approach is \textit{firing rules}, i.e., Datalog rules that capture successful and failed rule derivations. Firing rules for positive queries were first introduced in~\cite{kohler2012declarative}. These rules are similar to other query instrumentation techniques that have been used for provenance capture such as the rewrite rules of Perm~\cite{GM13}. One of our major contributions is to extend this concept for negation and failed rule derivations which is needed to support \datalogneg and missing answers.
Firing rules provide sufficient information for constructing explanations. However, to make this approach efficient, we need to avoid capturing rule derivations that will not contribute an explanation, i.e., they are not connected to $\provQ$ %user question 
atoms in the provenance graph. We achieve this by propagating information from the  $\provQ$ %user question 
throughout the query to prune rule derivations early on 
1) if they do not agree with the constants in the question 
%(e.g., in the running example, $\rel{Q}(n,s)$ can only be
%connected to derivations %instantiations 
%of rule $r_1$ with $X = n$ and $Y = s$)
%$\provQ$ %user question 
or 2) if we can determine that based on their success/failure status they cannot be part of the explanations. 
%(e.g., only successful derivations are connected to the node representing an existing result tuple). 
For instance, in the running example, $\rel{Q}(n,s)$ can only be
connected to successful derivations %instantiations 
of rule $r_1$ with $X = n$ and $Y = s$.
We then construct a graphical representation of the
explanation (e.g., the graphs shown in this paper were produced by our
implementation). 
Importantly, most parts of the Datalog program are independent of the requested provenance type. 
Only the last step (step 5 in Section~\ref{sec:compute-gp})
%(constructing the edge relation of the provenance graph from information captured by the firing rules) 
varies depending on what type of provenance graph is requested. 
%based on the exsitence or absence 
%of the tuples in the database.
%Additionally, based on the user question, we may be able to predetermine that we
%are only interested in successful or failed %won or lost 
%states for certain nodes types (e.g., in the
%example for why $\rel{Q}(n,s)$, we are only interested in existing $\rel{Train}$ relation tuples).
%In addition, by simultaneously instantiating and solving the game, we avoid the
%execution of a non-stratified program and only create edges in the graph that
% TODO: good moves not introduced
%represent good moves.
%are relevant for the user questions.
%
In summary, our main contributions are: %of this work are:
%
\begin{itemize}%[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
\item We demonstrate that the recently introduced provenance game model can
      serve as a unified framework for provenance of queries with
      negation and why-not provenance.
\item We present a type of provenance graph that are equivalent to provenance games, but more user friendly.
\item We extend the concept of firing rules to support negation and missing answers. 
  %    Furthermore, we discuss the relationship of these models to provenance and missing answer approaches.
\item We present an efficient approach computing the explanation
      for a  $\provQ$ %($\whyq Q(t)$ or $\whynotq Q(t)$) %a why or why-not questions 
      with  Datalog based on firing rules.
      Unlike the solution introduced in~\cite{KL13}, our approach
      %exploits information encoded in the question
      % For example, based on the constants in $t$ only certain nodes can be
      % connected to $Q(t)$ in the PG.
      %and 
      avoids unnecessary work by focusing the computation of relevant parts of a provenance graph.  % simultaneously instantiating and solving the explanations.% , solving, and restriction to
      % % TODO: 'good moves not introduced'
      % ``good moves''.
% \item We demonstrate that provenance games generalize m-semiring provenance,
%       an extension of the semiring framework for set difference and, thus,
%       negation.
%       We also prove that by extending semirings with annotations of partial
%       semiring expressions which encode relevant parts of the input Datalog
%       program, both model become equivalent.
%       Since a semirings have only been define for relational algebra queries,
%       this requires a translation between non-recursive \Datalogneg and positive
%       relational algebra extended with set-difference (we use $\RAplusminus$ to
%       denote this version of relational algebra).
%\item We generate Datalog program using firing rules for both positive queries and queries with negation
%      to capture only relevant explanations to the user's $\provQ$. 
      %by extending the technique (firing rules capturing successful derivations) 
      %to support computing failed derivations, and thus provide unified framework.  
% \item We formally prove the correctness of our algorithm for computing the
%       explanations for the user's $\provQ$. % and study its runtime complexity.
      % Interestingly, while the solution introduced in~\cite{KL13} runs in
      % \textsc{PTime} in the size of the active domain and in \textsc{ExpTime} in 
      % the number of variables per rule, our approach's runtime only depends on
      % the size of the instance (which may be exponentially more compact) for
      % games without negation and for queries with negation is bound by a smaller
      % exponential factor (the number of existential variables in rules for
      % missing tuples).
\item We present a full implementation of our approach in the GProM~\cite{AG14} system.
      %(Generic Provenance Middleware) 
      Using this system, we compile Datalog into relational algebra, optimizes the resulting algebra
      expressions, and translate optimized expressions into SQL code that
      can be executed by a standard relational database backend.
      % for every answer and non-answer to $Q$. 
      % Furthermore, given  we discuss how to directly compute GP restricted to
      % parts necessary for answering the users query.  Specifically, the user
      % questions enforces a particular structure on the game.
% \item We discuss how to derive other types of provenance from provenance 
%       games.\BG{Will we?}
\end{itemize}
\BG{Not sure about the last one, but I think we can also compute Ade's Why-not
    style provenance from the GP}
\vspace{-0.5mm}
%The remainder of the paper is organized as follows.
%In Section~\ref{sec:rel-work}, we discuss related work and
%% and provide necessary background in Section~\ref{sec:background}.
% introduce %provenance games in Section~\ref{sec:gp} and demonstrate
%how to compute explanations %provenance games 
%efficiently in Section~\ref{sec:compute-gp}.
%% In Section~\ref{sec:rel-to-others} we prove the equivalence of game provenance
%% and an extension of the semiring framework with set difference.
%% We present an experimental evaluation of our prototype implementation in
%% Section~\ref{sec:experiments} and conclude in Section~\ref{sec:concl}.
%We present our implementation in
%Section~\ref{sec:transl-into-relat}, discuss experimental results in
%Section~\ref{sec:experiments}, and conclude in Section~\ref{sec:concl}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "2016_GameProM"
%%% End:


==> prolog_sty.tex <==
\makeatletter

% initialisation of user macros
\newcommand\PrologPredicateStyle{}
\newcommand\PrologVarStyle{}
\newcommand\PrologAnonymVarStyle{}
\newcommand\PrologAtomStyle{}
\newcommand\PrologOtherStyle{}
\newcommand\PrologCommentStyle{}

% useful switches (to keep track of context)
\newif\ifpredicate@prolog@
\newif\ifwithinparens@prolog@

% save definition of underscore for test
\lst@SaveOutputDef{`_}\underscore@prolog

% local variables
\newcount\currentchar@prolog

\newcommand\@testChar@prolog%
{%
  % if we're in processing mode...
  \ifnum\lst@mode=\lst@Pmode%
    \detectTypeAndHighlight@prolog%
  \else
    % ... or within parentheses
    \ifwithinparens@prolog@%
      \detectTypeAndHighlight@prolog%
    \fi
  \fi
  % Some housekeeping...
  \global\predicate@prolog@false%
}

% helper macros
\newcommand\detectTypeAndHighlight@prolog
{%
  % First, assume that we have an atom.
  \def\lst@thestyle{\PrologAtomStyle}%
  % Test whether we have a predicate and modify the style accordingly.
  \ifpredicate@prolog@%
    \def\lst@thestyle{\PrologPredicateStyle}%
  \else
    % Test whether we have a predicate and modify the style accordingly.
    \expandafter\splitfirstchar@prolog\expandafter{\the\lst@token}%
    % Check whether the identifier starts by an underscore.
    \expandafter\ifx\@testChar@prolog\underscore@prolog%
      % Check whether the identifier is '_' (anonymous variable)
      \ifnum\lst@length=1%
        \let\lst@thestyle\PrologAnonymVarStyle%
      \else
        \let\lst@thestyle\PrologVarStyle%
      \fi
    \else
      % Check whether the identifier starts by a capital letter.
      \currentchar@prolog=65
      \loop
        \expandafter\ifnum\expandafter`\@testChar@prolog=\currentchar@prolog%
          \let\lst@thestyle\PrologVarStyle%
          \let\iterate\relax
        \fi
        \advance \currentchar@prolog by 1
        \unless\ifnum\currentchar@prolog>90
      \repeat
    \fi
  \fi
}
\newcommand\splitfirstchar@prolog{}
\def\splitfirstchar@prolog#1{\@splitfirstchar@prolog#1\relax}
\newcommand\@splitfirstchar@prolog{}
\def\@splitfirstchar@prolog#1#2\relax{\def\@testChar@prolog{#1}}

% helper macro for () delimiters
\def\beginlstdelim#1#2%
{%
  \def\endlstdelim{\PrologOtherStyle #2\egroup}%
  {\PrologOtherStyle #1}%
  \global\predicate@prolog@false%
  \withinparens@prolog@true%
  \bgroup\aftergroup\endlstdelim%
}

% language name
\newcommand\lang@prolog{Prolog-pretty}
% ``normalised'' language name
\expandafter\lst@NormedDef\expandafter\normlang@prolog%
  \expandafter{\lang@prolog}

% language definition
\expandafter\expandafter\expandafter\lstdefinelanguage\expandafter%
{\lang@prolog}
{%
  language            = Prolog,
  keywords            = {},      % reset all preset keywords
  showstringspaces    = false,
  alsoletter          = (,
  alsoother           = @$,
  moredelim           = **[is][\beginlstdelim{(}{)}]{(}{)},
  MoreSelectCharTable =
    \lst@DefSaveDef{`(}\opparen@prolog{\global\predicate@prolog@true\opparen@prolog},
}

% Hooking into listings to test each ``identifier''
\newcommand\@ddedToOutput@prolog\relax
\lst@AddToHook{Output}{\@ddedToOutput@prolog}

\lst@AddToHook{PreInit}
{%
  \ifx\lst@language\normlang@prolog%
    \let\@ddedToOutput@prolog\@testChar@prolog%
  \fi
}

\lst@AddToHook{DeInit}{\renewcommand\@ddedToOutput@prolog{}}

\makeatother
%
% --- end of ugly internals ---


% --- definition of a custom style similar to that of Pygments ---
% custom colors
\definecolor{PrologPredicate}{RGB}{000,031,255}
\definecolor{PrologVar}      {RGB}{024,021,125}
\definecolor{PrologAnonymVar}{RGB}{000,127,000}
\definecolor{PrologAtom}     {RGB}{186,032,032}
\definecolor{PrologComment}  {RGB}{063,128,127}
\definecolor{PrologOther}    {RGB}{000,000,000}

% redefinition of user macros for Prolog style
\renewcommand\PrologPredicateStyle{\color{PrologPredicate}}
\renewcommand\PrologVarStyle{\color{PrologVar}}
\renewcommand\PrologAnonymVarStyle{\color{PrologAnonymVar}}
\renewcommand\PrologAtomStyle{\color{PrologAtom}}
\renewcommand\PrologCommentStyle{\itshape\color{PrologComment}}
\renewcommand\PrologOtherStyle{\color{PrologOther}}

% custom style definition 
\lstdefinestyle{Prolog-pygsty}
{
  language     = Prolog-pretty,
  upquote      = true,
  stringstyle  = \PrologAtomStyle,
  commentstyle = \PrologCommentStyle,
  literate     =
    {:-}{{\PrologOtherStyle :-}}2
    {,}{{\PrologOtherStyle ,}}1
    {.}{{\PrologOtherStyle .}}1
}

==> relation-to-others.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relation to the Semiring Annotation Framework}\label{sec:rel-to-others}

We now demonstrate the close relationship between game provenance and the semiring annotation framework plus its extension to set difference (and thus negation). It has been proven in~\cite{KL13} that provenance polynomials can be computed from game provenance for positive queries. We extend this result to queries with negation and semirings with monus. This translation leads to an novel approach for computing Why-not provenance using semirings with monus. Game provenance encodes additional information that is not encoded in provenance polynomials (m-semiring polynomials): 1) the order of goals is encoded in the game provenance, but not in provenance polynomials. For example, $p \times q = q \times p$ for provenance polynomials. However, in game provenance $p \times q$ and $q \times p$ can be distinguished, because the tuples node for $p$ (respective $q$) would be connected to a different goal node. 2) Game provenance explicitly encodes relevant parts of the datalog program whereas in the (m-)semiring model the annotations encode no information of about the program that generated a particular results. Thus, it is not possible to compute game provenance from m-semiring annotations. However, we  demonstrate how m-semirings can be extended with annotations on parts of a m-semiring annotation that encode rule applications and that the thus extended m-semirings are equivalent to game provenance. Formally, such annotations on semiring-annotations can be represented as functions from a semiring $\cal K$ to $\cal K$ as was demonstrated by Karvonarakis~\cite{K09}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Positive Queries and Provenance Polynomials}
\label{sec:pos-to-N[X]}

For completeness, we now repeat the results for positive queries and provenance polynomials.  As proven, for positive Datalog
programs $Q$, the semiring provenance polynomials as defined in
\cite{green2007provenance,grigoris-tj-simgodrec-2012} for atoms $A(\bar x) \in Q(D)$ can be derived from the solved instantiated game.

\mypara{Semiring Provenance Polynomials} Semiring provenance
\cite{green2007provenance,grigoris-tj-simgodrec-2012} attaches provenance
information to EDB and IDB facts. The provenance information are elements of a
commutative semiring $K$. A commutative semiring is an algebraic structure with
two distinct associative and commutative operations ``\KPlus'' and ``\KTimes''.
During query evaluation, result facts are annotated with elements from $K$ that
are created by combining the provenance information from input facts. For
example, in the join \rel{ R(a,b) \la S(a,b), T(a) } with \rel{S(a,b)} being
annotated with $p_1 \in K$ and \rel{T(a)} being annotated with $p_2 \in K$, the
result fact \rel{R(a,b)} will be annotated with $p_1 \KTimes p_2$. Intuitively,
``\KTimes'' is used to combine provenance information of \emph{joint} use of
input facts, whereas ``\KPlus'' is used for alternative use of input facts.

Depending on the conrete semiring used, different (provenance)
information is propagated during query evaluation. The \emph{most
  informative}\footnote{In the sense that for any other semiring $K'$,
  there exists a semiring homomorphism $\mathcal H : \NX
  \rightarrow K'$.  This has important implications in
  practice \cite{green2007provenance,grigoris-tj-simgodrec-2012}.}
semiring is the \emph{positive algebra provenance semiring}
$\NX$ \cite{green2007provenance,grigoris-tj-simgodrec-2012}
whose elements are polynomials with variables from a set $X$ and
coefficients from $\mathbb{N}$.  The operators ``\KTimes'' and
``\KPlus'' in $\NX$ are the usual addition and multiplication of
polynomials. Usually, facts from the input database $D$ are annotate
by variables from a set $X$. Formally, we use $\tj^{\NX}$ as a
function that maps a ground atom to its provenance annotation in \NX.
%

\mypara{Obtaining Semiring Polynomials from Game Provenance} 
%
%
Consider only positive programs, and fix an atom $A(\bar x)$ with $A(\bar x)\in
Q(D)$.
%
The provenance graph $\gprov_\ProgD{}{\D}(\mskol{A}{\bar x}) = (V,M,\glabel)$ for $A(\bar x)$ can easily
be transformed into an operator tree for a provenance polynomial. 
The operator tree is represented as a DAG $G^\OP(A(\bar x))$ in which common sub-expressions are re-used.
$G^\OP(A(\bar x)) = (V',M',\delta)$ has nodes $V'$, edges $M'$, and node labels
$\delta$. For a fixed $A(\bar x)$, the structures of $\gprov$ and $G^{\OP}$ coincide, that is
$V=V'$ and $M=M'$.
The labeling function $\delta$ maps inner nodes to either ``$+$'' or ``$\KTimes$'', 
denoting n-ary versions of the semiring operators.
%
%
Leaf nodes in game provenance graphs correspond to atoms over the EDB schema. We
here only assign elements from $K$ to leaf nodes of the form $\mskol{r_R}{\bar x}$. 
%
%
Formally, the labeling function $\delta$ is defined as follows:
%

%
\begin{equation}\label{eq:simpleL}
  \delta(v) = 
  \begin{cases}
     \tj^{\NX}(A(\bar x)) &\textnormal{if }\;\;  \Flr(v) = \emptyset
     \;\textnormal{ and }\; v = \mskol{r_A}{\bar x}\\
     \mbox{``$\KTimes$''} &\textnormal{if }\;\;  \Flr(v) \neq \emptyset
     \;\textnormal{ and }\; \glabel(v)=\lost \\ 
     \mbox{``$\KPlus$''}  &\textnormal{if }\;\;  \Flr(v) \neq \emptyset
     \;\textnormal{ and }\; \glabel(v)=\won \\ 
  \end{cases}
\end{equation}
We use $\OP$ to denote the transformation of obtaining 
$G^\OP(A(\bar x))$ from $\gprov_\ProgD{}{\D}(\mskol{A}{\bar x})$. 
The provenance semiring polynomial of fact $A(\bar x)$ 
is now explicit in $G^\OP(A(\bar x))$. An
inner node ``$+$'' (or ``$\KTimes$'') with $n$ children represents an $n$-ary
version of $+$ (or $\KTimes$) from the semiring. Since the semiring operators are associative
and commutative, their $n$-ary versions are well-defined.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Proposition}
  For positive $Q$, and $A(\bar x)\in \Q(\D)$, all leaves in
  $\gprov_\ProgD{}{\D}(A(\bar x))$ are of type $\mskol{r_B}{X,Y}$;
  thus the labeling described above is complete.

\normalfont{\mypara{Sketch}
For positive programs, positive relation nodes are reachable from other positive
relation nodes over a path of length four as shown on the left side of \figref{fig-game-overview}.
For an atom $A(\bar x)\in Q(D)$, all reachable rule nodes are lost and all reachable goal nodes are 
won.}
\end{Proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The following theorem relates semiring provenance polynomials to the provenance
expressions we obtain in $G^{\OP}$:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{thm:poly}%
  Let $\gprov_\ProgD{}{\D}$ be the game provenance of an \RAplus query $Q$
  (in the form of a positive, non-recursive Datalog program) over database $D$.
Then  $\gprov_\ProgD{}{\D}$  represents the provenance
  polynomials \NX as follows:  for all $A(\bar x)\in Q(D)$,
 %
 \begin{displaymath}
   \OP\circ\gprov_\ProgD{}{\D}(\,\mskol{A}{\bar x}\,) \equiv
   \tj^\NX_\ProgD{}{\D}(\,A(\bar x)\,)  .
 \end{displaymath}

\normalfont{
\mypara{Sketch} %
Our game graph construction is an extension of the graph presented in Section 4.2 of 
\cite{grigoris-tj-simgodrec-2012}. Rule nodes 
correspond to the join nodes presented in \cite{grigoris-tj-simgodrec-2012}.
Named goal nodes can be seen as labels on the edges between (goal) tuple nodes and join nodes 
and allow us to identify at which position a tuple was used in the body.
For a detailed proof, please refer to Appendix \ref{sec:Proof}.
}
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \setlength{\tabcolsep}{0.2em}
 \renewcommand{\arraystretch}{1.1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}[tp]
  \centering
\subfloat[Input database $D$]{
  \mbox{\resizebox{.35\columnwidth}{!}{\input{figures/hop.dot.tex}}}
  \label{hopgraph}
}
\hfill
   \subfloat[Labels $\delta$ for leaf nodes of $\gprov_\PHopD$. ] {
     \parbox[b][][t]{.28\textwidth}{  %
       \centering
       \begin{tabular}{|cc|c|c|}
       %
       \multicolumn{2}{|c|}{\textsf{\scriptsize hop}} & node $n$ & ~$\delta(n)$~ \\\hline
       %
       a & a & $\mskol{r_{hop}}{a,a}$ & $p$ \\
       a & b & $\mskol{r_{hop}}{a,b}$ & $q$ \\
       b & a & $\mskol{r_{hop}}{b,a}$ & $r$ \\
       b & c & $\mskol{r_{hop}}{b,c}$ & $s$ \\
       \end{tabular}
     }
     \label{3hopinputannotations}
   }    
   \hfill
   %
   \subfloat[${\NX}$-Provenance of $\mskol{3Hop}{a,a}$.] {
     \parbox[b][][t]{.56\textwidth}{ %
       \centering
       \begin{tabular}{|cc|c|c|c|c|c|c|}
       %
       \multicolumn{2}{|c|}{\textsf{\scriptsize 3hop}} & node $n$ &
       $\tj^{\NX}_\PHopD(n)$ \\\hline
        a & a & $\mskol{3Hop}{a,a}$  & $p^3+2pqr$ \\
        %
       \end{tabular}
     }
     \label{33hopan}
   }

  
\subfloat[$\gprov(\,\mskol{3Hop}{a,a}\,)$]{
  \mbox{\resizebox{.52\columnwidth}{!}{\input{figures/ThreeHop-goal-tgv.dot.tex}}}
 \label{3hopprovenance} 
}
\hfill
\subfloat[DAG $G^\OP = \OP \circ \gprov(\mskol{3Hop}{a,a}).\quad\;$ Interpreting
   $G^{\OP}$ yields  $p^3+2pqr$. ]{
  \mbox{\resizebox{.42\columnwidth}{!}{\input{figures/ThreeHop-goal-tgv-op.dot.tex}}}
  \label{3hopprovenanceOmega}
}
   
  \caption{\small Input graph for program \PHop in (a) using edge labeling according to (b). 
  Game provenance $\gprov_\PHopD$ for the query \rel{3Hop(a,a)} on input database of (a) is shown
  %
  in (d).
  When labeling leaf nodes according to (b), lost inner nodes by ``$\KTimes$'',
  and won inner nodes by ``$+$'' then the operator DAG $G^{\OP}$ shown in (e) is
  created. 
  This DAG represents the semiring-provenance polynomial for the query \rel{3Hop(a,a)} shown in
  (c) and .
  }
  \label{3hopprov}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}[Example \rel{\mathbf{3hop}} from~\cite{grigoris-tj-simgodrec-2012}]
$\;$ Consider the \rel{3Hop} query $\PHop$ used in Figure 7 of \cite{grigoris-tj-simgodrec-2012}:
\[
r_1: \quad \rel{3Hop}(X,Y) \,\Gets\, \rel{hop}(X,Z_1), \rel{hop}(Z_1,Z_2), \rel{hop}(Z_2,Y).
\]
The query uses an input database consisting of a single binary EDB relation
\rel{hop} representing a directed graph. It asks for pairs of nodes that are reachable
via exactly three edges(=\emph{hops}). 
An input database $D$ and $\tj^{\NX}_\PHopD$ annotations of \PHop are shown in
\figref{3hopinputannotations}.
%
%
\Figref{3hopprovenance} shows the game provenance $\gprov(\mskol{3Hop}{a,a})$ 
of fact \rel{3Hop(a,a)}. Positive won relation nodes indicate the existence of the corresponding fact 
in $\Prog{3Hop}(D)$. To obtain the provenance polynomial of fact $\mskol{3Hop}{a,a}$, 
we apply $\OP$ to $\gprov(\mskol{3Hop}{a,a})$ as shown in
\figref{3hopprovenanceOmega}: we replace inner won nodes by ``$\KTimes$'', inner
lost nodes by ``$+$'', and leaf nodes by their respective annotations from $K$
as given in \figref{3hopinputannotations} and \cite{grigoris-tj-simgodrec-2012}.
%
%
The so relabeled graph encodes the provenance equation
\[
  \OP\circ\gprov_\PHopD(\mskol{3Hop}{a,a}) = (p \KTimes p \KTimes p) \KPlus (p \KTimes q \KTimes r) \KPlus (p \KTimes q \KTimes r) 
                                       = p^3 \KPlus 2pqr
\]
which is equivalent to the annotation of provenance semiring polynomials as 
shown in \figref{33hopan} and \cite{grigoris-tj-simgodrec-2012}.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Negation and Monus-Semirings}
\label{sec:monus-sem}

In~\cite{GP10}, the authors extend the semiring annotation framework that was originally defined for positive relational algebra ($\RAplus$) to set difference and duplicate removal. Here we are only interested in the extension to set difference. To support set difference, the algebraic structure used to annotate tuples has to be extended with a new operation monus. The authors have studied what algebraic properties have to hold for this structure called m-semirings. Interestingly, the semiring of provenance polynomials ($\ProvPoly$) has to be extended to maintain its property as the most general form of semiring annotation. 
We use $\ProvMPoly$ to denote the resulting free structure for m-semirings  as defined in~\cite{GP10}. 

Let us start by illustrating the correspondence between game provenance and m-semiring provenance by means of an example. Consider again the relation $\rel{hop}(x,y)$ in \figref{hopgraph} and query $\PHop :=$
\begin{displaymath}
r_1: \quad \rel{3Hop}(X,Y) \,\Gets\, \rel{hop}(X,Z_1), \rel{hop}(Z_1,Z_2), \rel{hop}(Z_2,Y).
\end{displaymath}

Assume, we are asking for the provenance of $\neg \rel{3Hop(c,a)}$ or equivalently we could define a program $\PHop'$ with an additional rule $r_2$ shown below and ask for $\rel{not3Hop}(c,a)$. 
%
\begin{displaymath}
r_2: \quad \rel{not3Hop}(X,Y) \,\Gets\, \neg \rel{3Hop}(X,Y). 
\end{displaymath}

As explained before, Why-not questions, i.e., game provenance for a negated atom $\neg \rel{R}(\vec{X})$, can always be modeled as a Why-question over an extended program adding a rule $\rel{notR}(\vec{X}) \Gets R(\vec{X})$. Thus, in the following we will only consider Why-questions when discussing the equivalence of game provenance and m-semiring provenance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  \mbox{\resizebox{\columnwidth}{!}{\input{figures/ThreeHop-goal-neg-tgv.dot.tex}}}
  \caption{\small Why-not provenance for \rel{3Hop(c,a)} using provenance games.}
  \label{fig:3Hopprovneg}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Assume that the attributes of relation hop are named $A$ and $B$. Applying the translation schema from Section~\ref{sec:trans-dl-to-algebra} we can translate this program into the equivalent relational algebra expression $\translate{\rel{not3Hop}(X,Y)}$:

\begin{align*}
(\allDomain \times \allDomain) - \Pi_{X,Y} (\\
&\mathtab\rho_{X \gets A, Z_1 \gets B}(hop)
  \\&\bowtie \rho_{Z_1 \gets A, Z_2 \gets B}(hop) \\&\bowtie \rho_{z_2 \gets A, Y
    \gets B}(hop))
\end{align*}


Figure~\ref{fig:3Hopprovneg} shows $\gprov(\rel{not3Hop}(c,a))$, the provenance conditioned solved instantiated game for the Why-question $\rel{not3Hop}(c,a)$ over the instance from Figure~\ref{3Hopinputannotations}. Fact $\rel{not3Hop}(c,a)$ is explained by an successful application of rules $r_2$ which is caused by a  failure of rule $r_1$ to derive $\rel{3Hop}(c,a)$. This in turn is explained by all potential rule instantiations of $r_2$ failing. Each such failed grounding of $r_2$ is explained by the absence of one or more tuples from $\rel{Hop}$, which if added to the instance, would make this rule instantiation successful. For example, $r_1(c,a,a,a)$ corresponds to an hypothetical path of length three that starts in $c$ moves to $a$ and stays in $a$ through a self-loop. This path does not exist, because $(c,a)$ does not exist in the $\rel{Hop}$ relation. Note how the existing tuple $(a,a)$ is not included in $\gprov(\rel{not3Hop}(c,a))$, because it does not explain why $(c,a)$ is missing in $\rel{3Hop}(c,a)$.

Now consider the annotation on tuple $(c,a)$ in the result of evaluating the translated relational algebra expression $\translate{\rel{not3Hop}(X,Y)}$ under $\ProvMPoly$ m-semiring~\cite{GP10} semantics. Assume that $\allDomain = \{a,b,c\}$ and for simplicity assume all elements in the domain are annotated with the $1$ element of the semiring. Let us use $x_{a_1,a_2}$ to denote the variable annotating tuple $(a_1,a_2)$ in the hop relation, e.g., $X_{a,a} = p$ in Figure~\ref{3hopprov}. Here we divert from standard way of creating an abstractly tagged relation (a relation where each tuple is annotated with a distinct variable $x$) and also annotate tuples that do not exist in the instance with a variable. Usually, these tuples would just be annotated with the $0$-element of the semiring. However, for our purpose of explaining missing tuples, we require these annotations. Following these conventions the annotation of tuple $t = (c,a)$ in the result of query $\translate{\rel{not3Hop}(X,Y)}$ is:

\begin{align*}
Q(t) =  (1 \KTimes 1) - &( x_{c,a} \KTimes x_{a,a} \KTimes x_{a,a} \\
&\KPlus x_{c,a} \KTimes x_{a,b} \KTimes x_{b,a} \\
&\KPlus x_{c,a} \KTimes x_{a,c} \KTimes x_{c,a} \\
&\KPlus x_{c,b} \KTimes x_{b,a} \KTimes x_{a,a} \\
&\KPlus x_{c,b} \KTimes x_{b,b} \KTimes x_{b,a} \\
&\KPlus x_{c,b} \KTimes x_{b,c} \KTimes x_{c,a} \\
&\KPlus x_{c,c} \KTimes x_{c,a} \KTimes x_{a,a} \\
&\KPlus x_{c,c} \KTimes x_{c,b} \KTimes x_{b,a} \\
&\KPlus x_{c,c} \KTimes x_{c,c} \KTimes x_{c,a})
\end{align*}

Most of the $x_{a_1,a_2}$ variables are assigned to $false$, the $0$-element of semiring $\mathbb{B}$ if the $\ProvMPoly$ annotations are interpreted in $\mathbb{B}$. For example, $(a,b)$ is present in $\rel{hop}$ and, thus is annotated with $true$ (the 1-element of the semiring $\mathbb{B}$) whereas $(a,c)$ is not present and, thus, is annotated with $false$. If we evaluate this expression in the semiring $\mathbb{B}$ we get:

\begin{align*}
Q(t)^{\mathbb{B}} = (T \wedge T) \wedge \neg ( &(F \wedge T \wedge T) \\
\vee &(F \wedge T \wedge T)\\
\vee &(F \wedge F \wedge F)\\
%%%%%%%%%%
\vee &(F \wedge T \wedge T)\\
\vee &(F \wedge F \wedge T)\\
\vee &(F \wedge T \wedge F)\\
%%%%%%%%%%
\vee &(F \wedge F \wedge T)\\
\vee &(F \wedge F \wedge F)\\
\vee &(F \wedge F \wedge F)\\
)\\
= T &
\end{align*}

Note that $Q(t)$ can be computed from the instantiated game $\ginst(\rel{not3Hop}(c,a))$ (and, thus, also from the solved instantiated game $\gsol(\rel{not3Hop}(c,a))$) using an extension of the mapping for positive queries presented above. Specifically, we have to determine node labels by node type and not whether they are won or lost. This is because for positive queries the regular structure of the provenance conditioned solved game results in node labels being predetermined based on  node type. Furthermore, we need to consider nodes that are not in the provenance conditioned solved game, but only exist in the solved game. We modify the labelling function $\delta$ to a labelling function $\delta^M$ for negative queries as shown below:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}\label{eq:negationL}
  \delta^M(v) = 
  \begin{cases}
     \tj^{\NX}(A(\bar x)) &\textnormal{if } \Flr(v) = \emptyset \;\textnormal{ and }\; v = \mskol{r_A}{\bar x}\\
     \mbox{``$\KPlus$''} &\textnormal{if } v \textnormal{ is a positive goal}\\ 
     \mbox{``$\KTimes$''}  &\textnormal{if } v \textnormal{ is a rule node}\\ 
     \mbox{``$1\; -\; $''}  &\textnormal{if } v \textnormal{ is a negated goal}\\
     \mbox{``$\KPlus$''} &\textnormal{if } v \textnormal{ is a relation node}\\
  \end{cases}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We use $\Omega^M$ to denote the application of this labelling.
In this extended labelling, rule nodes correspond to multiplication, relation and positive goal nodes do to summation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{thm:polyM}%
  Let $\gprov_\ProgD{}{\D}$ be the provenance conditioned instantiated solved game of an \RAplusminus query $Q$
  (in the form of a positive, non-recursive Datalog program) over database $D$.
Then  $\gprov_\ProgD{}{\D}$  represents the provenance
  polynomials \NX as follows:  for all $A(\bar x)\in Q(D)$,
 %
 \begin{displaymath}
   \OP\circ\gprov_\ProgD{}{\D}(\,\mskol{A}{\bar x}\,) \equiv
   \tj^\NX_\ProgD{}{\D}(\,A(\bar x)\,)  .
 \end{displaymath}

\normalfont{
\mypara{Sketch} %
Our game graph construction is an extension of the graph presented in Section 4.2 of 
\cite{grigoris-tj-simgodrec-2012}. Rule nodes 
correspond to the join nodes presented in \cite{grigoris-tj-simgodrec-2012}.
Named goal nodes can be seen as labels on the edges between (goal) tuple nodes and join nodes 
and allow us to identify at which position a tuple was used in the body.
For a detailed proof, please refer to Appendix \ref{sec:Proof}.
}
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\BG{REMOVED: This expression can be created from the game provenance. Each sum
mand corresponds to a rule application (there are nine like there are nine rule application nodes in the GP). The difference to translations for positive programs into semiring expressions is that relation nodes have to be translated differently depending on whether node is used negated or not (whether its negation is connected to a goal node or the node itsef is connected to a goal node).
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Annotating Parts of the provenance polynomials with monus to encode game provenance structure}

To show equivalence of game provenance with monus semiring expressions we have to annotate parts of the monus provenance polynomials to encode the structure of the query and, thus, be able to derive the game provenance from the M-semiring expressions.

Such annotations can be added based on the structure of the input data log program rules (adding annotations for rules, goals, and idb relations). We can interpret these annotations as identity functions to not mess up the semantics of the expressions. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Computing Provenance Conditioned Solved Games from M-semiring Provenance}
\label{sec:m-semiring-to-GP}

Furthermore, to solve the game and determine the relevant subpart of the game graph (remove parts corresponding to bad moves) we have to evaluate the $\mathbb{N}[X]^{M}$ expression in the boolean semiring with monus $\mathbb{B}^{M}$. By traversing the expression top-down and observing boolean values for sub-expressions, we can determine the game provenance graphs (this is a way to figure out what are bad moves in the graph and, thus, which subgraphs should be removed from the game provenance).


Whether parts of the game provenance should be removed or not can be determined by studying the boolean values of parts of the $\mathbb{N}[X]^M$ expression and which immediate subexpressions influenced these parts. The rules for determining what parts we are interested in a top-down fashion can be stated for the individual operators based on which input influenced the output value.
These rules are shown in Figure~\ref{fig:rules-for-inclusion}.

\begin{figure*}[t]
  \centering
  \begin{tabular}{|l|c|cc|cc|}
    \hline
    Operator & Output & LeftIn & RightIn & LeftRelevant? & RightRelevant? \\ \hline
%%%%%%%%%%%%%%%%%%%%
    $\vee$ & \greenT & \greenT & \greenT & Yes & Yes \\ 
    & \greenT & \greenT & \redF & Yes & No \\ 
    & \greenT & \redF & \greenT & No & Yes \\ 
    & \redF & \redF & \redF & Yes & Yes \\ \hline
%%%%%%%%%%%%%%%%%%%% 
    $\wedge$ & \greenT & \greenT & \greenT & Yes & Yes \\ 
    & \redF & \greenT & \redF & No & Yes \\ 
    & \redF & \redF & \greenT & Yes & No \\ 
    & \redF & \redF & \redF & Yes & Yes \\ \hline
%%%%%%%%%%%%%%%%%%%%
    $\neg$ & \greenT & \redF & &Yes & \\
    & \redF & \greenT & &Yes & \\ \hline
  \end{tabular}
  
  \caption{Rules for determining whether to include parts into the game provenance}
\label{fig:rules-for-inclusion}
\end{figure*}


Consider a simpler example to see how this works out. 

\begin{align*}
  N2Hop(X,Y) &:- \neg 2Hop(X,Y)\\
  2Hop(X,Y) &:- Hop(X,Z), Hop(Z,Y)
\end{align*}

which translated gives us:

\begin{align*}
(\allDomain \times \allDomain) - \Pi_{X,Y}(
   \rho_{X \gets A, Z \gets B} (Hop) \times \rho_{Z \gets A, Y \gets B} (Hop)
)  
\end{align*}

Consider edb instance $Hop(a,b)$ and $Hop(b,b)$ and a question Why $N2Hop(a,a)$ we get the monus-semiring expression

\begin{align*}
  (d_1 \times d_1) - (
  x_{a,a} \times x_{a,a} + x_{a,b} \times x_{b,a}
)
\end{align*}

interpreting this expression in $\mathbb{B}^M$

\begin{align*}
  (\greenT \wedge \greenT) \wedge \neg ( 
(\redF \wedge \redF)
\vee (\greenT \wedge \redF)
)
\end{align*}

broken down into results for individual expressions:

\begin{align*}
  \greenT &= (\greenT \wedge \greenT) \wedge \neg ((\redF \wedge \redF) \vee (\greenT \wedge \redF))\\
\greenT &= (\greenT \wedge \greenT)\\
\greenT &= \neg ((\redF \wedge \redF) \vee (\greenT \wedge \redF))\\
\redF &= (\redF \wedge \redF) \vee (\greenT \wedge \redF)\\
\redF &=(\redF \wedge \redF) \\
\redF &= (\greenT \wedge \redF)\\
\end{align*}

Based on our rules the part of the provenance graph corresponding to $x_{a,b}$ should not be included because it did not influence the results of $x_{a,b} \times x_{b,a}$. In contrast $x_{a,a}$ should be included because it influenced the result of $x_{a,a} \times x_{a,a}$. Note that this reasoning should be applied top-down to determine which parts to exclude.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Ideas and Notes}

\textcolor{red}{One subtlety: in game provenance nodes are shared among subgraphs. This corresponds to the boolean circuits~\cite{DM14c} representation of provenance polynomials.}\\

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "2016_GameProM"
%%% End: 

